Probably Approximately Symmetric: Fast rigid Symmetry Detection with Global Guarantees

We present a fast algorithm for global rigid symmetry detection with approximation guarantees. The algorithm is guaranteed to find the best approximate symmetry of a given shape, to within a user-specified threshold, with very high probability. Our method uses a carefully designed sampling of the transformation space, where each transformation is efficiently evaluated using a sub-linear algorithm. We prove that the density of the sampling depends on the total variation of the shape, allowing us to derive formal bounds on the algorithm's complexity and approximation quality. We further investigate different volumetric shape representations (in the form of truncated distance transforms), and in such a way control the total variation of the shape and hence the sampling density and the runtime of the algorithm. A comprehensive set of experiments assesses the proposed method, including an evaluation on the eight categories of the COSEG data-set. This is the first large-scale evaluation of any symmetry detection technique that we are aware of.

==> background.tex <==
\section{Background}

A global symmetry can be defined by a transformation that maps the whole shape to itself. We will focus only on these symmetries here. Global symmetries can be further classified into Perfect and Imperfect Symmetries, where in perfect symmetry the shape should map exactly to itself whereas in imperfect symmetry the mapping should lead to error smaller than a user defined threshold. Comprehensive surveys on this topic, for shapes and images, can be found in \cite{mpwc_symmSurvey_12,Liu2010}.

There are efficient algorithms for perfect symmetry detection. For example, in the case of a collection of $n$ points, Atallah \cite{Atallah85} describe an $O(nlogn)$ algorithm for enumerating all axes of symmetry under reflection of a planar shape. Wolter {\em et al.} \cite{Wolter85} give exact algorithms, based on string matching, for detecting all rotational and involutional symmetries in point sets, polygons and polyhedra. The time complexities of the algorithms are shown to be $O(n)$ for polygons, $O(nlogn)$ for two- and three-dimensional point sets, and $O(n logn)$ time is also required for general polyhedra. These algorithms are sensitive to noise.

Sun {\em et al.} \cite{Sun1997} detect n-fold rotational symmetry based on the correlation of the extended Gaussian image [SS97].  Kazhdan {\em et al.} \cite{kazhdan2003symmetry} use Fourier methods to compute symmetry descriptors for data embedded in a voxel grid. Neither method comes with guarantees.

Martinet {\em et al.} \cite{martinet2006accurate} use generalized moments to detect symmetries in 3D shapes. They show that the extrema of these moments correspond to the axes of symmetries of the shape. Because the number of extrema points is a super set of the number of symmetries they need to verify each extrema point as a post-processing step of the algorithm. The authors claim that the method works well in practice but admit that nothing in the theory ensures that all extrema points are detected.

Analyzing symmetries by their generating transformations is not new. Zabrodisky {\em et al.} \cite{zabrodsky1995symmetry} proposed a symmetry distance and use it to measure imperfect symmetries. Their  symmetry distance measures the distance of a shape to the closest shape that is perfectly symmetric with respect to that transformation. Podolak {\em et al.} \cite{podolak2006planar} proposed a continuous symmetry with respect to every transformation within a given group, while Mitra {\em et al.} \cite{MitraGP06} vote for transformations that align boundary points with similar local shape descriptors. They assume a known transformation group, as we do, but contrary to this work they do not provide global approximation guarantees.

Kim {\em et al.} \cite{Kim:2010:MTF} propose a robust algorithm for the detection of global intrinsic symmetries in 3D surface meshes. The algorithm is based on the observation that symmetry invariant point sets can be detected robustly using critical points of the Average Geodesic Distance function.

Ovsjanikov {\em et al.} \cite{Ovsjanikov:2008:GIS} detect the global {\em intrinsic} symmetry of shapes by using the Global Point Signatures to transform intrinsic symmetries on the shape into extrinsic symmetries in a high dimensional signature space. 

Lipman \cite{LipmanCDF10} do not assume a given transformation group by introducing a symmetry factored embedding that factors out the symmetry and the Symmetry Factored Distance which is the Euclidean distance in the embedded space.  As a result, the problem of finding approximate and partial symmetries in a point set reduces to the problem of measuring connectedness in the correspondence graph and they use spectral methods to solve it. The algorithm finds approximate, as well as partial symmetries but does not provide global approximation guarantees.

%some possible references:
%
%Martinet's "Accurate Detection of Symmetries in 3D Shapes" - TOG 2006~\cite{martinet2006accurate}
%
%Funkhouser's "A Planar-Reflective Symmetry Transform for 3D Shapes" - TOG/SIGRAPH 2006~\cite{podolak2006planar}
%
%Lipman's "Symmetry factored embedding and distance" - TOG 2010~\cite{lipman2010symmetry}
%
%Cohen-Or's "A survey on shape correspondence" - CG Forum 2011~\cite{van2011survey}
%
%Mitra's "Discovering structural regularity in 3D geometry" - TOG 2008~\cite{pauly2008discovering}
%
%Zabrodsky's "Symmetry as a continuous feature" - PAMI 1995~\cite{zabrodsky1995symmetry}
%
%Kazhdan, Funkhouser and Rusinkiewicz's "Rotation invariant spherical harmonic representation of 3D shape descriptors" - - Eurographics 2003~\cite{kazhdan2003rotation}} 
